M^4I: Multi-modal Models Membership Inference

With the development of machine learning techniques, the attention of research has been moved from single-modal learning to multi-modal learning, as real-world data exist in the form of different modalities. However, multi-modal models often carry more information than single-modal models and they are usually applied in sensitive scenarios, such as medical report generation or disease identification. Compared with the existing membership inference against machine learning classifiers, we focus on the problem that the input and output of the multi-modal models are in different modalities, such as image captioning. This work studies the privacy leakage of multi-modal models through the lens of membership inference attack, a process of determining whether a data record involves in the model training process or not. To achieve this, we propose Multi-modal Models Membership Inference (M^4I) with two attack methods to infer the membership status, named metric-based (MB) M^4I and feature-based (FB) M^4I, respectively. More specifically, MB M^4I adopts similarity metrics while attacking to infer target data membership. FB M^4I uses a pre-trained shadow multi-modal feature extractor to achieve the purpose of data inference attack by comparing the similarities from extracted input and output features. Extensive experimental results show that both attack methods can achieve strong performances. Respectively, 72.5% and 94.83% of attack success rates on average can be obtained under unrestricted scenarios. Moreover, we evaluate multiple defense mechanisms against our attacks. The source code of M^4I attacks is publicly available at https://github.com/MultimodalMI/Multimodal-membership-inference.git.

==> 7_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets?
%   \answerTODO{}
%   %\answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\answerYes{} 
\item Did you describe the limitations of your work?
\answerYes{}
\item Did you discuss any potential negative societal impacts of your work?
\answerYes{We discussed the consequences of multi-modal model membership inference in the Introduction.}
\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
\answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
\item Did you state the full set of assumptions of all theoretical results?
\answerNA{We did not include theoretical results in this research.}
\item Did you include complete proofs of all theoretical results?
\answerNA{We did not include theoretical results in this research.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerYes{The source code of M$^4$I attacks  is publicly available at \url{https://github.com/MultimodalMI/Multimodal-membership-inference}. The URL is provided at the end of Abstract.}
\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
\answerYes{}
\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerNo{The results of multiple times of training will not affect the trend of the results, given limited computing resources.}
\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerYes{We provide the computation resource used in our experiment in Supplementary Materials.} 
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
\item If your work uses existing assets, did you cite the creators?
\answerYes{We cited all the existing assets used in this research, including code~\cite{opacus, chen-acl-2021-r2gencmn}, data~\cite{coco, young-etal-2014-image, iapr}, and models~\cite{vinyals2015tell}.}
\item Did you mention the license of the assets?
\answerYes{The license of the assets is provided in the Supplementary Materials.}
\item Did you include any new assets either in the supplemental material or as a URL?
\answerYes{The URL of M$^4$I source code is provided at the end of Abstract.}
\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerYes{}
\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNo{The three public datasets we used do not contain any personally identifiable information or offensive content.} 
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
\item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA{We did not use crowdsourcing or conduct research with human subjects.}
\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{We did not use crowdsourcing or conduct research with human subjects.}
\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
\answerNA{We did not use crowdsourcing or conduct research with human subjects.}
\end{enumerate}


\end{enumerate}
